The effect of cosmic web filaments on galaxy properties in the RESOLVE and ECO surveys

Galaxy environment plays an important role in driving the transformation of galaxies from blue and star-forming to red and quenched. Recent works have focused on the role of cosmic web filaments in galaxy evolution and have suggested that stellar mass segregation, quenching of star formation and gas-stripping may occur within filaments. We study the relationship between distance to filament and the stellar mass, colour and HI gas content of galaxies using data from the REsolved Spectroscopy of a Local VolumE (RESOLVE) survey and Environmental COntext (ECO) catalogue, two overlapping census-style, volume-complete surveys. We use the Discrete Persistence Structures Extractor (DisPerSE) to identify cosmic web filaments over the full ECO area. We find that galaxies close to filaments have higher stellar masses, in agreement with previous results. Controlling for stellar mass, we find that galaxies also have redder colours and are more gas poor closer to filaments. When accounting for group membership and halo mass, we find that these trends in colour and gas content are dominated by the increasing prevalence of galaxy group environments close to filaments, particularly for high halo mass and low stellar mass galaxies. Filaments have an additional small effect on the gas content of galaxies in low-mass haloes, possibly due to cosmic web stripping.

==> Introduction.tex <==
testing if this works as expected
